Multi-agent online learning in time-varying games

We examine the long-run behavior of multi-agent online learning in games that evolve over time. Specifically, we focus on a wide class of policies based on mirror descent, and we show that the induced sequence of play (a) converges to Nash equilibrium in time-varying games that stabilize in the long run to a strictly monotone limit; and (b) it stays asymptotically close to the evolving equilibrium of the sequence of stage games (assuming they are strongly monotone). Our results apply to both gradient-based and payoff-based feedback - i.e., the "bandit feedback" case where players only get to observe the payoffs of their chosen actions.

==> Algorithms/Restart.tex <==
%----------------------------------------------------------------------
%%% RESTART
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\tt
\begin{algorithmic}[1]
\Require
	Horizon $\nRuns$,
	batch size $\batch$,
	choice algorithm $\alg$ as in \eqref{eq:algo}
	\medskip
\State
	set $\run\leftarrow\start$
	\Comment{step counter}
\State
	choose $\state^{\start}\in\points$
	\Comment{initialization}
\Repeat
\State
%	set $\iBatch\leftarrow\floor{\run/\batch}+1$
	set $\tau\leftarrow \floor{(\run-1)/\batch}\batch + 1$
	\Comment{augment every $\batch$ stages}
	\State
		play $\state^{\run}\in\points$
		\Comment{play chosen action}
%	\State
%		receive $\pay^{\run}(\state^{\run})$ 
%		\Comment{collect reward}
	\State
		get signal $\signal^{\run}$
		\Comment{receive feedback}
	\State
		set $\state^{\run+1} \leftarrow \alg(\state^{\tau},\signal^{\tau},\dotsc,\state^{\run},\signal^{\run})$
		\Comment{update action}
	\State
		$\run\leftarrow\run+1$
		\Comment{next stage}
\Until{$\run>\nRuns$}
	\Comment{end play}
\end{algorithmic}

==> Algorithms/TVG.tex <==
%----------------------------------------------------------------------
%%% TIME-VARYING GAME
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{algorithmic}[1]
\Require
%	players $\play\in\players$,
%	action spaces $\points_{\play}\subseteq\R^{\vdim_{\play}}$
	sequence of stage games $\game_{\run} \equiv \game_{\run}(\players,\points,\pay_{\run})$
	\smallskip
\For{$\run=\running$}
	\For{$\play=1,\dotsc,\nPlayers$} \textbf{simultaneously}
%	\State
%		set $\game\leftarrow\game^{\run}(\players,\points,\pay^{\run})$
%		\Comment{stage game}
%	\ForAll{$\play\in\players$}
	\State
		play $\state_{\play,\run}\in\points_{\play}$
		\Comment{action selection}
	\State
		get $\pay_{\play,\run}(\state_{\run})$ 
		\Comment{receive reward}
	\State
		observe $\signal_{\play,\run}$
		\Comment{get feedback}
	\EndFor
\EndFor
\end{algorithmic}

==> Learning.tex <==
%----------------------------------------------------------------------
%%% LEARNING
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


%----------------------------------------------------------------------
%%% Mirror descent
%----------------------------------------------------------------------
\subsection{Mirror descent\afterhead}
\label{sec:mirror}

%----------------------------------------------------------------------
\beginrev

The most widely used method for no-regret learning is the family of algorithms known as \acdef{OMD}.
Viewed abstractly, the basic idea of the method is as follows:
\begin{enumerate*}
[(\itshape a\upshape)]
\item
each player $\play\in\players$ plays an action $\point_{\play}\in\points_{\play}$ and receives a gradient signal $\dvec_{\play} \in \dspace_{\play}$;
subsequently,
\item
each player takes an ``approximate gradient'' step from $\point_{\play}$ along $\dvec_{\play}$ to generate a new action $\new\point_{\play}$,
and the process repeats.
\end{enumerate*}
Formally, this can be written in recursive form as
\begin{equation}
\label{eq:prox-abstract}
\new\point_{\play}
	= \proxplay{\point_{\play}}{\step\dvec_{\play}}
\end{equation}
where:
\begin{enumerate}
\item
%$\proxmap_{\play} \from \dpoints_{\play} \to \points_{\play}$
$\proxmap_{\play}$
denotes the ``prox-mapping'' of player $\play$
%which determines the precise way in which the step along $\dpoint$ is taken
(discussed in detail below).
\item
$\step$ is a step-size parameter controlling the weight attributed to the signal $\dvec_{\play}$.
\end{enumerate}
The ``prox-scheme'' \eqref{eq:prox-abstract} will be our main focus in the sequel so some remarks are in order:

\begin{remark}
To streamline our presentation, we will often suppress the focal player index and write more simply
\begin{equation}
\label{eq:prox-abstract-noplay}
\new\point
	= \prox{\point}{\step\dvec}.
\end{equation}
As we explain below, this slight abuse of notation is justified by the fact that \eqref{eq:prox-abstract} can be seen equivalently as referring to the action profile $\point = (\point_{1},\dotsc,\point_{\nPlayers})$ of all players $\play\in\players$, with $\proxmap$ denoting the corresponding product map $\proxmap \defeq \prod_{\play}\proxmap_{\play}$.
The precise meaning of \eqref{eq:prox-abstract-noplay} will always be made clear from the context, so there is no danger of confusion.
\remend
\end{remark}

\endrev
%----------------------------------------------------------------------

\begin{remark}
The terminology ``descent'' alludes to the fact that the algorithm was originally stated in the framework of convex function minimization (as opposed to reward maximization).
In this context, methods based on \acl{MD} have received intense scrutiny ever since the pioneering work of \citet{NY83};
for an appetizer, see \citet{BecTeb03}, \citet{NJLS09}, \citet{Nes09}, \citet{SS11}, \citet{BCB12}, \citet{Teb18}, \citet{MZ19}, and references therein.
We should also mention here that ``\acl{OMD}'' is sometimes used synonymously with the popular \acdef{FTRL} protocol of \citet{SSS06}.
The two methods coincide in linear problems, but not otherwise;
in general, \ac{FTRL} requires access to a best-response oracle, so it is beyond the scope of this paper.
\remend
\end{remark}


To get some intuition about the method, the archetypal example of a prox-mapping is the Euclidean projector
\begin{flalign}
\prox{\point}{\dpoint}
	= \Eucl(\point + \dpoint)
	&\defeq \argmin_{\pointalt\in\cvx}
		\braces*{ \norm{\point +  \dpoint - \pointalt}_{2}^{2} }
%	\notag\\
	= \argmin_{\pointalt\in\cvx}
		\braces*{ \braket{\dpoint}{\point - \pointalt} + \tfrac{1}{2} \norm{\pointalt - \point}_{2}^{2} }
\label{eq:prox-Eucl}
\end{flalign}
\ie the closest-point projection of $\point + \dpoint$ onto a given convex  $\cvx$.
%\footnote{In writing $\point + \dpoint$, we are blurring the lines between primal and dual vectors.
%This distinction is reinstated in the second line of \eqref{eq:prox-Eucl} where $\dpoint\in\dspace$ is paired properly to $\point-\pointalt\in\vecspace$.}
Going beyond this familiar example, the key novelty of \acl{MD} is to replace the quadratic term in \eqref{eq:prox-Eucl} by the so-called \emph{Bregman divergence}
\begin{equation}
\label{eq:Bregman}
\breg(\pointalt,\point)
	= \hreg(\pointalt) - \hreg(\point) - \braket{\nabla \hreg(\point)}{\pointalt - \point},
\end{equation}
induced by a ``\acli{DGF}'' $\hreg$ on $\cvx$.
%This function plays the role of the squared Euclidean norm in \eqref{eq:Bregman-Eucl} and is known as a \acdef{DGF};
More precisely, in the spirit of \citet{JNT11}, we have the following definition:

\begin{definition}
\label{def:Bregman}
Let $\cvx$ be a compact convex subset of $\vecspace \cong \R^{\vdim}$.
%Let $\hreg\from\vecspace\to\R\cup\{\infty\}$ be a proper \ac{lsc} convex function on $\vecspace$.
We say that $\hreg\from\vecspace\to\R\cup\{\infty\}$ is a \acdef{DGF} on $\cvx$ if
\begin{enumerate}
%\addtolength{\itemsep}{\smallskipamount}
\item
$\hreg$ is proper, \ac{lsc} and convex.
\item
The effective domain of $\hreg$ is $\dom\hreg \defeq \setdef{\point\in\vecspace}{\hreg(\point) < \infty} = \cvx$.
\item
The subdifferential of $\hreg$ admits a \emph{continuous selection}:
specifically, writing
\begin{equation}
\label{eq:prox-domain}
\subcvx
	\defeq \dom\subd\hreg
	= \setdef{\point\in\cvx}{\subd\hreg(\point)\neq\varnothing}
\end{equation}
for the domain of $\subd\hreg$, there exists a continuous mapping $\nabla\hreg\from\subcvx\to\dspace$ such that $\nabla\hreg(\point) \in \subd\hreg(\point)$ for all $\point\in\subcvx$.
\item
$\hreg$ is $\hstr$-strongly convex relative to $\norm{\cdot}$, \ie
\begin{equation}
\label{eq:hreg-str}
\hreg(\pointalt)
	\geq \hreg(\point)
	+ \braket{\nabla\hreg(\point)}{\pointalt - \point}
	+ \tfrac{\hstr}{2} \norm{\pointalt - \point}^{2}
\end{equation}
for all $\point\in\subcvx$ and all $\pointalt\in\cvx$.
\end{enumerate}
Given a \ac{DGF} $\hreg$ on $\cvx$,
the \emph{Bregman divergence} $\breg\from\subcvx\times\cvx\to\R$ induced by $\hreg$ is given by \eqref{eq:Bregman},
and
the associated \emph{prox-mapping} $\proxmap\from\subcvx\times\dspace\to\subcvx$ is defined as
\begin{equation}
\label{eq:proxmap}
\prox{\point}{\dpoint}
	= \argmin_{\pointalt\in\cvx} \ \braces*{\braket{\dpoint}{\point - \pointalt} + \breg(\pointalt,\point)}
	\quad
	\text{for all $\point\in\subcvx$, $\dpoint\in\dspace$}.
\end{equation}
%for all $\point\in\subcvx$, $\dpoint\in\dspace$.
Finally, we say that $\hreg$ is \emph{Lipschitz} if $\sup_{\point\in\subcvx} \dnorm{\nabla\hreg(\point)} < \infty$.
\end{definition}
\smallskip

\begin{remark}
%In a slight abuse of notation,
For simplicity, when $\cvx$ is understood from the context, we will not distinguish between $\hreg$ and its restriction $\hreg\vert_{\cvx}$ on $\cvx$.
Also, because $\proxmap$ is defined only for $\point\in\subcvx$, the set $\subcvx = \dom\subd\hreg$ will be sometimes referred to as the \emph{prox-domain} of $\hreg$.
\remend
\end{remark}

Before continuing, it will be instructive to provide some standard examples of the above:
\medskip

\begin{example}
[Euclidean projections]
\label{ex:prox-Eucl}
We begin by revisiting Euclidean projections on some compact convex subset $\cvx$ of $\R^{\vdim}$.
Letting $\hreg(\point) = \frac{1}{2} \norm{\point}^{2}$ for $\point\in\cvx$, we readily see that $\subcvx=\cvx$;
moreover, $\nabla\hreg(\point) = \point$ is a continuous selection of $\subd\hreg(\point)$ for all $\point\in\cvx$.
Hence, the associated Bregman divergence is
\begin{equation}
\label{eq:Bregman-Eucl}
\breg(\pointalt,\point)
	= \tfrac{1}{2} \norm{\pointalt}_{2}^{2}
	- \tfrac{1}{2} \norm{\point}_{2}^{2}
	- \braket{\point}{\pointalt - \point}
	= \tfrac{1}{2} \norm{\pointalt - \point}_{2}^{2}.
\end{equation}
%and the induced prox-mapping is given by \eqref{eq:prox-Eucl}.
The resulting recursion $\new\point = \Eucl(\point + \step\dvec)$ is known as \acdef{OGD} and its no-regret properties were first established by \citet{Zin03}.
%and it was the first algorithm shown to achieve no regret by \citet{Zin03}.
\end{example}
\smallskip

\begin{example}
[Entropic regularization]
\label{ex:prox-entropic}
Let $\cvx = \simplex_{\vdim} \defeq \setdef{\point\in\R_{+}^{\vdim}}{\sum_{j=1}^{\vdim} \point_{j} = 1}$ denote the unit simplex of $\vecspace=\R^{\vdim}$.
A very widely used \acl{DGF} for this geometry is the (negative) \emph{Gibbs-Shannon entropy} $\hreg(\point) = \sum_{j=1}^{\vdim} \point_{j}\log\point_{j}$.
By inspection, the domain of subdifferentiability of $\hreg$ is $\subcvx \defeq \relint\cvx$, and the resulting Bregman divergence is just the \acdef{KL} divergence
\begin{equation}
\label{eq:Bregman-KL}
\breg(\pointalt,\point)
	= \dkl(\pointalt, \point)
	\defeq \sum_{j=1}^{\vdim} \pointalt_{j}\log\left(\frac{\pointalt_{j}}{\point_{j}}\right)
	\quad
	\text{for all $\point\in\subcvx$, $\pointalt\in\cvx$}.
\end{equation}
%valid for all $\point\in\subcvx$, $\pointalt\in\cvx$.
In turn, a standard calculation gives rise to the prox-mapping
\begin{equation}
\label{eq:prox-MW}
\prox{\point}{\dpoint}
	= \frac
		{(\point_{1}e^{\dpoint_{1}},\dotsc,\point_{n}e^{\dpoint_{n}})}
		{\point_{1}e^{\dpoint_{1}} + \dotsm + \point_{n}e^{\dpoint_{n}}}
\end{equation}
for all $\point\in\subcvx$, $\dpoint\in\dspace$.
%----------------------------------------------------------------------
\beginrev
The corresponding update rule $\new\point = \prox{\point}{\step\dvec}$ is widely known in optimization as \acli{EGD} \citep{BecTeb03,KW97}, and as the
\emph{``Hedge''} (or exponential/multiplicative weights) algorithm
%\acdef{MW} algorithm (or \emph{``Hedge''} or \emph{``exponential weights''})
in game theory and online learning \citep{Vov90,LW94,AHK12,FS99,ACBFS95}.
\endrev
%----------------------------------------------------------------------
\end{example}
\smallskip


%\begin{example}[Fermi-Dirac regularization]
%\label{ex:prox-FD}
%Let $\cvx=[0,1]$ and let $\hreg(\point) = \point\log(\point) + (1-\point)\log(1-\point)$ be the (negative) Fermi-Dirac entropy of $\point$.
%Then, $\subcvx = (0,1)$ and the induced prox-mapping is given by the expression
%\begin{equation}
%\label{eq:prox-FD}
%\prox{\point}{\dpoint}
%	= \frac{\point e^{\dpoint}}{1 - \point + \point e^{\dpoint}}
%	\quad
%	\text{for all $\point\in(0,1)$, $\dpoint\in\R$}.
%\end{equation}
%\end{example}
%\smallskip


%----------------------------------------------------------------------
\beginrev

Going back to our multi-agent setting, let $\game_{\run} \equiv \game_{\run}(\players,\points,\pay_{\run})$ be a sequence of stage games, and assume each player $\play\in\players$ is endowed with an individual \ac{DGF} $\hreg_{\play}\from\points_{\play}\to\R$ and corresponding prox-mapping $\proxmap_{\play} \from \subpoints_{\play} \times \dpoints_{\play} \to \subpoints_{\play}$, where $\subpoints_{\play} \defeq \dom\subd\hreg_{\play}$ and $\dpoints_{\play} \defeq \dspace_{\play}$.%
\footnote{We also write $\breg_{\play}$ for the Bregman divergence of player $\play$, and we assume that it is $\hstr_{\play}$-strongly convex.}
%and Bregman divergence $\breg_{\play}$.
We then obtain the general class of \emph{prox-learning} methods
\begin{equation}
\label{eq:proxplay}
\tag{PL$_{\play}$}
\state_{\play,\run+1}
	= \proxplay{\state_{\play,\run}}{\step_{\run} \signal_{\play,\run}},
\end{equation}
or, in more compact notation
\begin{equation}
\label{eq:prox}
\tag{PL}
\state_{\run+1}
	= \prox{\state_{\run}}{\step_{\run} \signal_{\run}}
\end{equation}
where:
\begin{enumerate}
[\indent 1.]
\addtolength{\itemsep}{.5ex}
\item
$\run=\running$ denotes the stage of the process.
\item
$\state_{\run} = (\state_{\play,\run})_{\play\in\players}$ denotes the players' action profile at stage $\run$.
%For concreteness, we also assume throughout that $\state_{\run}$ is initialized at the so-called ``prox-center'' $\point_{c} \defeq \argmin\hreg$ of $\points$.
\item
$\signal_{\run} = (\signal_{\play,\run})_{\play\in\players}$ denotes the signals received by the players at stage $\run$, assumed throughout to be provided by an oracle of the general form \eqref{eq:signal}.
\item
$\step_{\run} > 0$ is a (nonincreasing) step-size sequence.
\item
The \emph{collective} (or aggregate) prox-mapping $\proxmap \defeq \prod_{\play}\proxmap_{\play} \from\subpoints\times\dpoints\to\subpoints$ is defined as $\prox{\point}{\dpoint} = (\proxplay{\point_{\play}}{\dpoint_{\play}})_{\play\in\players}$ for all $\point \in \subpoints \defeq \prod_{\play} \subpoints_{\play}$ and all $\dpoint \in \dpoints \defeq \prod_{\play}\dpoints_{\play}$.
%with each individual prox-mapping $\proxmap_{\play}\from\subpoints_{\play}\times\dpoints_{\play}\to\points_{\play}$ derived from a player-specific \acl{DGF} $\hreg_{\play}\from\points_{\play}\to\R$.%
%\footnote{Specifically, for $\point = (\point_{1},\dotsc,\point_{\nPlayers}) \in \points$ and $\dpoint = (\dpoint_{1},\dotsc,\dpoint_{\nPlayers}) \in \dpoints$, we have $\prox{\point}{\dpoint} = (\proxmap_{\play}(\point_{\play},\dpoint_{\play}))_{\play\in\players}$.}
%Naturally, the product map $\proxmap$ is induced by the \ac{DGF} $\hreg(\point) = \sum_{\play\in\players} \hreg_{\play}(\point_{\play})$.}
\end{enumerate}
Unless explicitly mentioned otherwise, all learning policies described in the sequel will be of the form above;
for a pseudocode implementation, see \cref{alg:prox}.

\endrev
%----------------------------------------------------------------------


%----------------------------------------------------------------------
%% Prox algorithm begins here

\begin{algorithm}[t]
\small
\ttfamily
\caption{Prox-learning
\hfill
\small
[player indices suppressed]}
\input{Algorithms/Prox}
\label{alg:prox}
\end{algorithm}

%% Prox algorithm ends here
%----------------------------------------------------------------------


%----------------------------------------------------------------------
\beginrev

%----------------------------------------------------------------------
%%% Regret minimization
%----------------------------------------------------------------------
\subsection{Regret minimization\afterhead}
\label{sec:no-reg-stat}

We now proceed to state the no-regret properties of the class of prox-learning algorithms under study.
To that end, it will be useful to employ the following gap functions for a sequence of actions $\state_{\run} \in \points$:
\begin{subequations}
\label{eq:gap}
\begin{align}
\label{eq:gap-point}
\gap_{\point_{\play}}(\runs)
	&= \sum_{\run\in\runs} \braket{\vecfield_{\play,\run}(\state_{\run})}{\point_{\play} - \state_{\play,\run}}
\shortintertext{and}
\label{eq:gap-max}
\gap_{\play}(\runs)
	&= \max_{\point_{\play}\in\points_{\play}} \gap_{\point_{\play}}(\runs).
%	&= \max_{\point\in\points} \sum_{\run\in\runs} \braket{\vecfield_{\run}(\state_{\run})}{\point - \state_{\run}}.
\end{align}
\end{subequations}
Given that each $\pay_{\play,\run}$ is assumed individually concave in $\point_{\play}$,
%\footnote{Since we are suppressing the player index $\play\in\players$, the above refers to the \emph{individual} concavity of each player's payoff function.}
we have
\begin{flalign}
\pay_{\play,\run}(\point_{\play};\state_{-\play,\run}) - \pay_{\play,\run}(\state_{\play,\run};\state_{-\play,\run})
	&\leq \braket{\vecfield_{\play,\run}(\state_{\play,\run};\state_{-\run})}{\point_{\play} - \state_{\play,\run}}
	\notag\\
	&\leq \braket{\vecfield_{\play,\run}(\state_{\run})}{\point_{\play} - \state_{\play,\run}}
\end{flalign}
for all $\point_{\play}\in\points_{\play}$ and all $\run\in\runs$.
As a result, the regret incurred by the $\play$-th player under $\state_{\run}$ can be upper bounded as
\begin{equation}
\label{eq:reg-gap-stat}
\reg_{\play}(\runs)
	\leq \gap_{\play}(\runs)
\end{equation}
\ie $\gap_{\play}(\runs)$ can be used as a direct proxy for minimizing the player's regret.
\Cref{prop:gap} below provides a precise technical statement to that effect:

\begin{proposition}
\label{prop:gap}
Suppose that player $\play\in\players$ runs \cref{alg:prox} over the interval $\runs = \window{\runstart}{\nRuns}$ with
%a \acl{DGF} such that $\breg_{\points} \equiv \sup_{\point,\pointalt} \breg(\point,\pointalt) < \infty$,
%and
oracle feedback of the form \eqref{eq:signal}.
%Then, over any window of the form $\runs = \{\runstart,\runstart+1,\dotsc,\runstart+\nRuns\}$, we have:
Then:
\begin{equation}
\label{eq:gap-bound}
\gap_{\point_{\play}}(\runs)
%	\leq \frac{\breg_{\points}}{\step_{\nRuns}}
	\leq \sum_{\run\in\runs} \parens*{\frac{1}{\step_{\run}} - \frac{1}{\step_{\run-1}}} \breg_{\play}(\point_{\play},\state_{\play,\run})
%	\leq \sum_{\run\in\runs} \frac{\breg(\point,\state_{\run+1}) - \breg(\point,\state_{\run})}{\step_{\run}}
	+ \sum_{\run\in\runs} \braket{\error_{\play,\run}}{\state_{\play,\run} - \point_{\play}}
	+ \frac{1}{2\hstr_{\play}} \sum_{\run\in\runs} \step_{\run} \dnorm{\signal_{\play,\run}}^{2}
\end{equation}
with the convention $\step_{\runstart-1} = \infty$.
Moreover, if $\step_{\run}$ is non-increasing, we also have
\begin{equation}
\label{eq:gap-mean-bound}
\exof{\gap_{\play}(\runs)}
%	\leq \frac{\breg_{\points}}{\step_{\nRuns}}
	\leq 2\sum_{\run\in\runs} \parens*{\frac{1}{\step_{\run}} - \frac{1}{\step_{\run-1}}} \dbound_{\play,\run}
	+ 2\diam(\points_{\play}) \! \sum_{\run\in\runs} \bbound_{\play,\run}
	+ \frac{1}{2\hstr_{\play}} \sum_{\run\in\runs} \step_{\run}
		\totbound_{\play,\run}^{2}
%		(\sbound_{\play,\run}^{2} + \sdev_{\play,\run}^{2})
\end{equation}
where $\dbound_{\play,\run} = \exof{\max_{\point_{\play}\in\points_{\play}} \breg_{\play}(\point_{\play},\state_{\play,\run})}$.

\end{proposition}

Using this bound (which we prove in \cref{app:regret}), we obtain the following guarantee:

%\begin{theorem}
%\label{thm:reg-stat}
%Suppose that \cref{alg:prox} is run
%by player $\play\in\players$
%with a step-size of the form $\step_{\run} \propto \run^{-\pexp}$, $\pexp\in[0,1]$,
%a Lipschitz \acl{DGF},
%and feedback of the form \eqref{eq:signal} with $\bbound_{\run} = \bigoh(1/\run^{\bexp})$ and $\totbound_{\run}^{2} = \bigoh(\run^{2\sexp})$ for some $\bexp,\sexp \geq 0$.
%Then, the player's regret is bounded as
%\begin{equation}
%\label{eq:reg-play}
%\exof{\reg_{\play}(\nRuns)}
%	= \tilde\bigoh\parens*{\nRuns^{\pexp} + \nRuns^{1-\bexp} + \nRuns^{1+2\sexp-\pexp}}.
%\end{equation}
%In particular, if the algorithm is run with $\step_{\run} \propto \run^{-1/2}$ and unbiased \ac{SFO} feedback with finite variance \textpar{$\bexp = \infty$, $\sexp = 0$}, we have:
%%for $\pexp=(1-\vexp)/3$, we obtain the optimized bound
%\begin{equation}
%\label{eq:reg-mean-dyn-tuned}
%\exof{\reg_{\play}(\nRuns)}
%	= \tilde\bigoh\parens[\big]{\nRuns^{1/2}}.
%\end{equation}
%\end{theorem}

\begin{theorem}
\label{thm:reg-stat}
Suppose that \cref{alg:prox} is run
by player $\play\in\players$
with constant step-size $\step >0$ and oracle feedback of the form \eqref{eq:signal}.
Then, the regret incurred by the player is bounded as
\begin{equation}
\label{eq:reg-mean-stat}
\exof{\reg_{\play}(\runs)}
	\leq \frac{2\depth_{\play}}{\step}
	+ 2\diam(\points_{\play}) \sum_{\run\in\runs} \bbound_{\play,\run}
	+ \frac{\step}{2\hstr_{\play}} \sum_{\run\in\runs} \totbound_{\play,\run}^{2}
\end{equation}
where
$\depth_{\play} \defeq \max\hreg_{\play} - \min\hreg_{\play}$ denotes the ``depth'' of $\hreg_{\play}$ over $\points_{\play}$.
\end{theorem}

\begin{corollary}
\label{cor:reg-stat}
Suppose that the focal player's oracle feedback is unbiased and bounded in mean square, \ie $\bbound_{\play,\run} = 0$ and $\totbound_{\play,\run}^{2} \leq \totbound^{2}$ for some $\totbound < \infty$.
If \cref{alg:prox} is run with step-size $\step = (2/\totbound) \sqrt{\hstr\depth/\nRuns}$ for some $\depth \geq \depth_{\play}$, $\hstr \leq \hstr_{\play}$, the player's regret is bounded as
\begin{equation}
\label{eq:reg-mean-stat-unbiased}
\exof{\reg_{\play}(\nRuns)}
	\leq 2\totbound \sqrt{(\depth/\hstr)\nRuns}.
\end{equation}
%Finally, if the oracle is perfect \textpar{$\error_{\run} = 0$ for all $\run$}, we have
%\begin{equation}
%\label{eq:reg-mean-stat-perfect}
%\reg_{\play}(\nRuns)
%	\leq 2\vbound \sqrt{(\depth/\hstr)\nRuns}.
%\end{equation}
\end{corollary}

%\begin{remark}
%In the perfect oracle case ($\error_{\run} = 0$ for all $\run$), the bound \eqref{eq:reg-mean-stat-unbiased} can be tightened by a factor of $\sqrt{2}$ to $\reg_{\play}(\nRuns) \leq \vbound \sqrt{(2\depth/\hstr)/\nRuns}$;
%this plays no role in the sequel.
%\end{remark}

Bounds of this type are fairly common in online optimization \citep{CBL06,SS11,BCB12} and justify the characterization ``no-regret learning'' for the class of algorithms under study.
That being said, we haven't been able to find a precise reference for the impact of the oracle's bias on the regret, so, for completeness, we provide a proof of \cref{thm:reg-stat} in \cref{app:regret}.
\smallskip

We should also note that \Cref{thm:reg-stat} makes no assumptions about the behavior of all other players $\playalt\neq\play$ in the game:
they could behave arbitrarily, even to the detriment of their individual interests (as encoded by their payoff functions).
In particular, their actions could even adapt to the actions of the focal player:
in this case, \cref{thm:reg-stat,cor:reg-stat} still hold as stated,
but the notion of regret is less meaningful as a figure of merit.

\cref{thm:reg-stat} also leaves open the question whether \cref{alg:prox} provides any guarantees for \emph{dynamic} regret minimization.
We address this question in the context of our game-theoretic analysis in the next section.

\endrev
%----------------------------------------------------------------------
